Scaling Autoregressive Multi-Modal Models: Pretraining and Instruction Tuning

We present CM3Leon (pronounced "Chameleon"), a retrieval-augmented, token-based, decoder-only multi-modal language model capable of generating and infilling both text and images. CM3Leon uses the CM3 multi-modal architecture but additionally shows the extreme benefits of scaling up and tuning on more diverse instruction-style data. It is the first multi-modal model trained with a recipe adapted from text-only language models, including a large-scale retrieval-augmented pre-training stage and a second multi-task supervised fine-tuning (SFT) stage. It is also a general-purpose model that can do both text-to-image and image-to-text generation, allowing us to introduce self-contained contrastive decoding methods that produce high-quality outputs. Extensive experiments demonstrate that this recipe is highly effective for multi-modal models. CM3Leon achieves state-of-the-art performance in text-to-image generation with 5x less training compute than comparable methods (zero-shot MS-COCO FID of 4.88). After SFT, CM3Leon can also demonstrate unprecedented levels of controllability in tasks ranging from language-guided image editing to image-controlled generation and segmentation.

==> notes.tex <==

\paragraph{Text-Guided Image Editing:} This task encompasses generating altered images based on an initial image and text-based instructions. These instructions may involve adjustments to seasonal and weather conditions, background substitutions, alterations to material attributes, and conversion of artistic mediums, among other modifications. Following the methodology of instructpix2pix(\citep{instructpix2pix}), we processed their data using proprietary face-filtering techniques, resulting in approximately 600,000 examples.

\paragraph{Image-to-Image Grounded Generation (8 tasks):} This task empowers the user to generate grounding images, utilizing various image features and text prompts. Such image features include edge maps, segmentation maps, key points, and human poses. These can be extracted from user-uploaded images or the user's sketches. We meticulously curated 7 million examples using ControlNet(\citep{controlnet}) processing code, extracting features such as canny edge, hed boundary, user sketching, human pose, uniform segmentation, Midas depth, Midas 3D norm map, and MLSD line from Shutterstock datasets.

\paragraph{Spatially Grounded Image Generation:} This task facilitates the user in incorporating spatial information into text prompts to produce images (For instance: "Fabricate an image of a contemporary kitchen with a refrigerator at the location (50, 50) -> (120, 200), and stoves at the location (140, 120) -> (200, 160)"; "Create a high-definition image of {caption} with {bbox+label}, and {bbox+label}"). Drawing from the work on pix2seq(\citep{pix2seq}), each object is represented by discrete tokens, encompassing the bounding box's coordinates [ymin, xmin, ymax, xmax] and a class label. We employed widely recognized object detection datasets like MS-COCO(\cite{mscoco}), Openimage(\cite{openimage}), and Object365(\cite{object365}), assembling 3 million training examples.

\paragraph{How-to-write:} This task allows the user to ask the model to write signs or logos based on a text prompt. We use OCR detector to find suitable examples from Shutterstock datasets. We prepared 200,000 such examples. 


\begin{figure}[H]
\vspace{-3em}
    \centering
    \begin{tabular}{cc}
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/cm3leon_octopus.png}
        \end{subfigure}
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/koala_bear.png}
        \end{subfigure}
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/astronaut_horse.png}
        \end{subfigure}
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/teddy_bear.png}
        \end{subfigure}
        \\
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/red_beret_gsd.png}
        \end{subfigure}
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/astr_armenian_church.png}
        \end{subfigure}
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/khachkar_forest_poms.png}
        \end{subfigure}
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/cat_sunglasses.png}
        \end{subfigure}
        \\
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/cactus_straw_hat.png}
        \end{subfigure}
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/hand.png}
        \end{subfigure}
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/racoon_samurai.png}
        \end{subfigure}
        \begin{subfigure}{0.15\textwidth}
    \includegraphics[width=\textwidth]{graphics/showcase_0/1991_anime.png}
        \end{subfigure}
        \\
    \end{tabular}
    \caption{Showcase of \model{} zero-shot generations (no-retrieval augmentation). For full list of prompts refer to \ref{sec:showcase_prompts}.}
    % \caption{\small \olga{Zero-shot (?) text-to-image generations with \model{} model. Prompts used for image generation,} Top to Bottom, Left to Right: \textit{Chameleon and octopus, side by side, high quality render, drawing, professional.}, \textit{A plush toy koala bear relaxing on a lounge chair and working on a laptop. The chair is beside a rose flower pot. There is a window on the wall beside the flower pot with a view of snowy mountains.}, \textit{A photo of an astronaut riding a horse in the forest. There is a river in front of them with water lilies.}, \textit{A teddy bear wearing a motorcycle helmet and cape is riding a motorcycle in Rio de Janeiro with Dois Irmãos in the background. dslr photo.}}
\end{figure}


\section{Related Work}
The core domain most related to our work is text-to-image generation.
\paragraph{Diffusion Models}
Significant progress in the domain of text-to-image generation has been achieved through the use of diffusion models \citep{LDM, GLIDE, DALLE2}. %The underlying mechanism involves sequentially adding noise to an image and then learning to reverse the noise based on provided text inputs or features \citep{unified_perspective_diffusion}. 
Diffusion models generally incorporate pre-trained text or language representations such as the text encoder of the CLIP \citep{CLIP} image-text model or text encoders like T5 \citep{T5}. The recursive application of multi-resolution diffusion model (by employing multiple steps of super-resolution) has further enhanced their capability to generate high-quality images from text prompts, leading to state-of-the-art zero-shot non-retrieval based MS-COCO FID scores \citep{IMAGEN}.

\paragraph{Retrieval Augmented Diffusion Models}
Conventional text-to-image models often struggle to capture the vast array of concepts and entities in the image domain. Methods like enabling retrieval during inference time can help address the complexity of these tail entities by delegating it to a retrieval step. Building on the work of \citet{IMAGEN}, \citet{REIMAGEN} incorporates retrieval to enhance zero-shot MS-COCO FID scores, demonstrating further improvement in this area.

\paragraph{Autoregressive Token Models}
Significant advancements have been made in the field by utilizing large language models over tokenized image representations \citep{taming, DALLE}. A widely-used approach in the field \citep{vqvae,vqvae2,vqvae_gan} involves an initial stage of converting images into discrete latent variables through tokenization. Consequently, this transforms text-to-image generation into a sequence-to-sequence problem, which transformer-based language models can effectively address. This approach enables the straightforward application of techniques and insights from large language models to learn text-to-image generation models \citep{DALLE, makeascene}.

\paragraph{Non-Autoregressive Token Models}
Although autoregressive models have benefited from extensive research in NLP, their autoregressive decoding makes them slow. Non-autoregressive models, such as \citet{maskpredict}, have been proposed in NLP and extended to text-to-image models, exemplified by \citet{MUSE} which achieves state-of-the-art image generation performance and higher efficiency than diffusion or autoregressive models by employing masked modeling in discrete token space (non-autoregressively with iterative decoding).

\paragraph{Retrieval Augmented Autoregressive Token Models}
Token-level models face challenges akin to those encountered by non-retrieval augmented diffusion models. To address these issues, \citet{RA_CM3} suggested prefixing decoder-only text-to-image models, such as \citet{DALLE, CM3}, with statically retrieved instances during training, resulting in significant efficiency gains during the training process. Our paper primarily concentrates on the implementation of this particular strategy.

\section{Appendix Clone}
\section{Pre-Training}
\subsection{Data Visualizations}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{graphics/cm3leon_single_image.drawio.pdf}
    \caption{Visualization of the tokenization of one caption-image pair.}
    \label{fig:single_image_tokenization}
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{graphics/cm3leon_multiple_image.drawio.pdf}
    \caption{Visualization of the tokenization of a full training sample consisting of retrieved sampled and query caption-image pair. \arunb{may be different color for <eos> and <break> ?} \vasu{maybe use different colors or text to demarcate which image-text pair comes from which source} \binh{for consistency with Figure 2, perhaps we can also use multiple boxes (e.g. 2 small ones) to represent Text and Image}}
    \label{fig:multiple_image_tokenization}
\end{figure}
\subsection{Model Hyper-Parameters}
\begin{table}[h]
\centering\small
\begin{tabular}{l|cccccccc}
\toprule
Model size & \#~L & d$_{\text{model}}$ & Seq Length & Batch & LR & Warmup Steps & \#~GPUs & \#~Tokens \\
\midrule
350M   & 24  & 1024  & 4096      & 8M & 6e-04     & 1500  & 256  & 1.4T      \\
760M  & 24  & 1536  & 4096      & 8M & 5e-04     & 1500  & 256 & 1.9T    \\
7B    & 32  & 4096 & 4096      & 8M & 1.2e-04     & 1500   & 512 & 2.4T      \\
\bottomrule
\end{tabular}
\caption{{\bf Model architecture details.}  We report the
number of layers (\#~L), embedding size (d$_{\text{model}}$), sequence length, batch size, peak learning rate (LR), learning rate warmup steps, number of GPUs used, and number of tokens consumed by each model.}
\label{tab:pretraing_para}
\end{table}
\section{Inference Latency and Throughput}
\begin{figure}[htbp]
  \centering
  \begin{minipage}[c]{0.49\textwidth}
    \centering\small
    \begin{tabular}{lcc}
    \toprule
    Model & Resolution & Time \\
    \midrule
    Imagen & $256 \times 256$ & 9.1s  \\
    Imagen & $1024 \times 1024$ & 13.1s  \\
    LDM (50 steps) & $512 \times 512$ & 3.7s \\
    LDM (250 steps) & $512 \times 512$ & 18.5s \\
    Parti (3B) & $256 \times 256$ & 6.4s \\
    MUSE (3B) & $256 \times 256$ & 0.5s \\
    CM3Leon (7B, BF16) & $256 \times 256$ & 11.8s \\
    CM3Leon (7B, INT8) & $256 \times 256$ & 9.1s \\
    \bottomrule
    \end{tabular}
    \caption{\small Inference latency for several models.}
    \label{tab:inference-tine}
  \end{minipage}
  \hfill
  \begin{minipage}[c]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{graphics/inference_perf/new_inference_throughput.pdf}
  \caption{Inference throughput of \model{}-7B for generating images, without retrieval, across different model parallelism (MP), FasterTransformer (FT) implementation, data type (DType) and batch sizes}\label{fig:inference_perf}
  \end{minipage}
\end{figure}
\binh{The numbers in \autoref{tab:inference-tine} are taken from \cite{MUSE} (they also copied LDM numbers from \href{https://lambdalabs.com/blog/inference-benchmark-stable-diffusion}{this blog}). Assuming these numbers are for batch size 1 and MP1, it might be hard to argue at inference time our model is more efficient than Parti or even Stable Diffusion / LDM? Our 7B model is certainly much larger than the rest, though.}

\section{Supervised Fine Tuning}
\subsection{Hyper-Parameters}\label{sec:sft_hp}
To maintain a balanced dataset during training, we implemented an up/down sampling strategy with a threshold of 3/0.3.  This process was executed on the 760M and 7B models using 64 and 128 80GB A100s, respectively. We assembled our training examples into sequences of length 4096. Preliminary experiments were conducted to identify optimal learning rates from a range of ${ 1\mathrm{e}{-5}, 3\mathrm{e}{-5}, 5\mathrm{e}{-5}, 1\mathrm{e}{-4}}$ and per-GPU batch sizes from ${4, 8, 16}$ using our validation split. The selected hyperparameters are cataloged in Table \ref{tab:sft_para}. Throughout the fine-tuning phase, our models processed approximately 30 billion tokens.
\begin{table}[h]
\centering\small
\begin{tabular}{l|cccccc}
\toprule
Model & \#~GPUS & Seq Length & Batch Size & LR & Warm-up Steps & \#~Tokens \\
\midrule
CM3Leon-760m  & 64 & 4096        & 2M & 5e-05     & 150    & 30B      \\
CM3Leon-7b   & 128  & 4096      & 2M & 5e-05     & 150    & 30B      \\
\bottomrule
\end{tabular}
\caption{Fine-tuning parameters for \model{} models }
\label{tab:sft_para}
\end{table}
\subsection{Training Data Breakdown}
\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{p{0.2\textwidth}|p{0.65\textwidth}|p{0.12\textwidth}}
\toprule
Dataset & Template &  \# Examples \\
\midrule
\multicolumn{3}{c}{Image Focused Datasets} \\
\midrule
InstructPix2Pix & Edit first image following the instruction [break] \{image1\} [break] {edit instruction} [break] \{image 2\} & 127k \\[0.5cm]

OCR & draw ``\{ocr\_content\}'' [break] \{image\} & 300k \\[0.5cm]

Object Detection & Generate high quality image of \{caption\} with segmentations \{obj1\} at \{loc1\}, \{obj2\} at \{loc2\} ... [break] \{image\} & 3M \\[0.5cm]

Edge-to-Image & Make high quality image from canny edge features [break] \{edge image\} [break] \{caption\} [break] \{image\} & 1M \\[0.5cm]

Seg-to-Image & Make high quality image from a segmentation map [break] \{seg image\} [break] \{caption\} [break] \{image\} & 1M \\[0.5cm]

Hed-to-Image & Make high quality image from hed features [break] \{seg image\} [break] \{caption\} [break] \{image\} & 1M \\[0.5cm]

Pose-to-Image & Make high quality image from openpose features [break] \{seg image\} [break] \{caption\} [break] \{image\} & 142k \\[0.5cm]

Depth-to-Image & Make high quality image from depth features [break] \{depth image\} [break] \{caption\} [break] \{image\} & 1M \\[0.5cm]

Norm-to-Image & & 1M \\[0.5cm]

Scribbe-to-Image & Make high quality image from children's scribbles [break] \{scribble image\} [break] \{caption\} [break] \{image\} & 500k \\

\midrule
\multicolumn{3}{c}{Text Focused Datasets} \\
\midrule

\makecell[l]{COCO Captioning \\ \citep{chen2015microsoft}} & \makecell[l]{\{caption\} [break] \{image\} \\ Describe the given picture. \{caption\} [break] \{image\} \\ } & 591k \\[0.5cm]

\makecell[l]{Flickr30k \\ \citep{young2014image}} & \makecell[l]{\{caption\} [break] \{image\} \\ Describe the given picture. \{caption\} [break] \{image\} \\ } & 144k \\[0.5cm]

\makecell[l]{Image Paragraph \\ \citep{krause2017hierarchical}} & \makecell[l]{Describe the given picture in very detail. \{caption\} [break] \\ \{image\} \\ Describe all the objects in the given image in very detail. \\ \{caption\} [break] \{image\} \\ Generate a long caption for the given image. \\ \{caption\} [break] \{image\} } & 14k \\[0.5cm]

\makecell[l]{Localized Narratives \\ \citep{pont2020connecting}} & \makecell[l]{Describe the given picture in very detail. \{caption\} [break] \\ \{image\} \\ Generate a long narration of what is happening in the \\ given image. \{caption\} [break] \{image\} \\ Generate a long caption for the given image. \\ \{caption\} [break] \{image\} } & 164k \\[0.5cm]

\makecell[l]{VQA2 \\ \citep{goyal2017making}} & \makecell[l]{Question: \{question\} Answer: \{answer\}. [break] {image} \\ Question: \{question\} [newline] \{answer\} [break] {image} \\ Question: \{question\} The answer is \{answer\}. [break] {image} } & 1.3M \\[0.5cm]

\makecell[l]{VizWiz \\ \citep{gurari2018vizwiz}} & \makecell[l]{Question: \{question\} Answer: \{answer\}. [break] {image} \\ Question: \{question\} [newline] \{answer\} [break] {image} \\ Question: \{question\} The answer is \{answer\}. [break] {image} } & 92k \\[0.5cm]

\makecell[l]{OKVQA \\ \citep{marino2019ok}} & \makecell[l]{Question: \{question\} Answer: \{answer\}. [break] {image} \\ Question: \{question\} [newline] \{answer\} [break] {image} \\ Question: \{question\} The answer is \{answer\}. [break] {image} } & 26k \\[0.5cm]

\makecell[l]{ScienceQA \\ \citep{lu2022learn}} & \makecell[l]{ Question: \{question\} [newline] Context: \{context\} [newline] \\ Options: \{choices\_text\} [newline] Answer: \{answer\}.  \\  Question: \{question\} [newline] Context: \{context\} [newline] \\ Options: \{choices\_text\} [newline] Answer: Let's think \\ step-by-step: \{ explanation\} So the answer is \{answer\}. } & 6k \\[0.5cm]

\bottomrule
\end{tabular}
} 
\caption{Details of the datasets and their prompt templates used in our supervised fine-tuning of \model{} models.}
\label{tab:sft-datasets}
\end{table}
\subsection{More Qualitative Samples}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{graphics/instruct_image_gen/sft examples.pdf}
    \vspace*{-5mm}
     \caption{Qualitative examples of finetuned CM3Leon-7b model.
    \label{fig:sft_image}
    }
\end{figure}
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{graphics/instruct_image_gen/caption_qa_examples.pdf}
    \vspace*{-5mm}
     \caption{Qualitative examples showing our SFT-\model{}-7B model's generations for image captioning and visual question answering tasks. 
    \label{fig:caption_vqa_examples}
    }
\end{figure}

Table~\ref{tab:models-summary} and Figure~\ref{fig:how_we_scale} provide a comparative overview of CM3Leon and various cutting-edge text-to-image models, evaluated based on the zero-shot MS-COCO (30K) task using the Fréchet Inception Distance (FID) as the primary metric. Notably, the CM3Leon-7B model establishes a new benchmark with an impressive FID score of 4.88.

Despite the utilization of larger training datasets and increased computational resources by models such as Stable Diffusion V1.5 (a diffusion-based model), and MUSE and PARTI (encoder-decoder models), their FID scores remain higher than that of CM3Leon, as Figure~\ref{fig:how_we_scale} reveals. This observation underlines the effectiveness of retrieval-augmented decoder-only models like CM3Leon. In particular, the CM3Leon-7B model, when operated with zero or one retrieved examples during inference, records superior FID scores. This result demonstrates the crucial role retrieval plays in expanding the model's world knowledge and its capacity to generate high-quality images. Remarkably, CM3Leon surpasses all other retrieval-augmented models, including KNN-diffusion and RE-IMAGEN.
